A CNN-based Prediction-Aware Quality Enhancement Framework for VVC

This paper presents a framework for Convolutional Neural Network (CNN)-based quality enhancement task, by taking advantage of coding information in the compressed video signal. The motivation is that normative decisions made by the encoder can significantly impact the type and strength of artifacts in the decoded images. In this paper, the main focus has been put on decisions defining the prediction signal in intra and inter frames. This information has been used in the training phase as well as input to help the process of learning artifacts that are specific to each coding type. Furthermore, to retain a low memory requirement for the proposed method, one model is used for all Quantization Parameters (QPs) with a QP-map, which is also shared between luma and chroma components. In addition to the Post Processing (PP) approach, the In-Loop Filtering (ILF) codec integration has also been considered, where the characteristics of the Group of Pictures (GoP) are taken into account to boost the performance. The proposed CNN-based Quality Enhancement(QE) framework has been implemented on top of the VVC Test Model (VTM-10). Experiments show that the prediction-aware aspect of the proposed method improves the coding efficiency gain of the default CNN-based QE method by 1.52%, in terms of BD-BR, at the same network complexity compared to the default CNN-based QE filter.

==> bdrates.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
						
	&	CNN-arch	&	Conf. Journal		year		Paper		&	Codec	&	CCN	&	Inter or Intra	&	In-loop Out-loop	&	Training dataset	&	Loss function Bit-depth	&	QP	&	Coding information	\\
\hline
1	&	MFRNet	&	arXiv 	-	2020	\cite{	ma2020mfrnet	}	&	VVC HEVC	&	48	&	One for both	&	In-loop 	&	BVI-DVC	&	L1-10	&	QP-specific	&	QP	\\
2	&	VRCNN	&	MMM	-	2020	\cite{	dai2017convolutional	}	&	HEVC	&	4	&	intra	&	Out-loop	&	-	&	L2	&	QP-specific	&	QP	\\
7	&	EDCNN	&	IEEE-TIP	-	2020	\cite{	pan2020efficient 	}	&	HEVC	&	37	&	both	&	In-loop	&	CTC-test sequences	&	L2+L1	&	ALLQPs	&	QP	\\
8	&	BSTN	&	MIPR	-	2020	\cite{	meng2020bstn 	}	&	HEVC	&		&	Both-LD, AI	&	Out-Loop	&	Derf’s collection SJTU dataset	&	L2	&	QP-Specific	&	TU-mean mask	\\
10	&	FGTSN	&	DCC	-	2020	\cite{	meng2020flow 	}	&	HEVC	&	10	&	both	&	Out-Loop	&	-	&	L2	&	QP-Specific	&	QP	\\
12	&	Residual-blocks	&	IEEE access	-	2020	\cite{	chen2020neural 	}	&	HEVC	&	20	&	both	&	Out-Loop	&	JCT-VC	&	L2	&	QP-Specific	&	QP	\\
17	&	-	&	arXiv 	-	2020	\cite{	lam2020efficient 	}	&	VVC	&		&	both	&	Out-Loop	&	CLIC	&	L2	&	QP-map	&	QP	\\
24	&	-	&	IEEE-TIP	-	2020	\cite{	liu2020comprehensive 	}	&HEVC	&	-	&	-	&		&	LUI	&		&		&		\\
25	&	FQE-CNN	&	  IEEE-TCSVT	-	2020	\cite{	 huang2020frame	}	&	HEVC	&	58	&	Intra	&	Out-Loop	&	ADE20K, DIV2K, CLIC	&	L2	&	QP	&	QP Intra Mode Map	\\
30	&	-	&	ICME	-	2020	\cite{	zhang2020enhancing 	}	&	VVC	&	34	&	RA	&	Out-Loop	&	BVI-HFR BVI-Texture Harmonic 4K Netflix Chimera	&	L1	&	QP-Specific	&	QP	\\
38	&	RBQE	&	arXiv 	-	2020	\cite{	xing2020early 	}	&	HEVC	&	25	&	AI	&	Out-loop	&	RAISE	&	L2	&	ALL QP	&	QP	\\
39	&		&	arXiv 	-	2020	\cite{	strumpler2020learning 	}	&	JPEG	&		&		&		&		&		&		&		\\
41	&	IFN-ND \ PQEN-ND	&	Neurocomputing 	-	2020	\cite{	sun2020quality 	}	&	HEVC	&68	&	AI and P	&	In-loop	&	SJTU 4 K xiph.org	&	L1	&	All QP	&	QP	\\
42	&	QEVC	&	ICCCS	-	2020	\cite{	li2020qevc 	}	&	HEVC	&	22	&	LD-RA	&	In-loop Out-loop	&	CDVL – REDS database	&	-	&	QP-Specefic	&	QP Motion estimation	\\
48	&	MSGDN	&	CVPRW	-	2020	\cite{	li2020multi 	}	&	VVC	&		&	intra	&	Out-Loop	&	COCO2014	&	L1 perceptual loss Adversarial loss	&	37 and 39	&	QP	\\
49	&	PMVE	&	IEEE-TC	-	2020	\cite{	ding2020biprediction 	}	&	HEVC	&		&	Inter-intra	&	Out-loop	&	-	&	L1 L2	&	QP- as input	&	QP	\\
50	&	MWGAN	&	arXiv 	-	2020	\cite{	wang2020multi 	}	&	HEVC	&		&	LD	&	Out-loop	&		&	L2, adversarial loss, motion loss, wavelet loss all based on L2	&	One QP	&	QP	\\
58	&	STEFCNN	&	DCC	-	2020	\cite{	xu2020spatial 	}	&	HEVC	&		&		&		&		&		&		&		\\
61	&		&	arXiv 	-	2020	\cite{	wang2020combining	}	&		&		&		&		&		&		&		&		\\
63	&	MPRNET	&	Neurocomputing 	-	2020	\cite{	jin2020post 	}	&	HEVC	&	19	&	AI	&	in-Loop	&	BSD500	&	ML-MSE loss, adversarial loss, and perceptual adversarial loss	&	QP-Specific	&	QP	\\
64	&	RRDB	&	UCET	-	2020	\cite{	wang2020visual	}	&	HEVC	&	29	&	AI	&	Out-Loop	&	BSDS500	&	GAN	&	QP-Specific	&	QP	\\
22	&	ADCNN	&	IEEE access	-	2019	\cite{	wang2019attention	}	&	VVC	&	40	&	Intra and Inter	&	In-Loop	&	DIV2K Xiph.org SJTU 4K	&	L1	&	QP-map	&	QP map CU map	\\
3	&	M-PRN	&	ICIP	-	2019	\cite{	wang2019partition	}	&	HEVC	&	68	&	AI	&	Out-loop	&	DIV2K	&	L2	&	QP-specific	&	QP- Multi-scale Mean value of CU (MM-CU)	\\
15	&	MFQE.2	&	 IEEE-TPAMI	-	2019	\cite{	guan2019mfqe	}	&	HEVC	&		&		&	Out-loop	&		&	L2	&	QP-Specific	&		\\
16	&	SDTS	&	ICIP	-	2019	\cite{	meng2019enhancing 	}	&	VVC	&		&	both	&	Out-Loop	&		&	L2	&	QP-Specific	&	QP	\\
18	&	VRCNN-BN	&	IEEE access	-	2019	\cite{	zhao2019cnn	}	&	HEVC	&	6	&	both	&	Out-Loop	&		&	L2	&		&		\\
19	&	MIF	&	IEEE-TIP	-	2019	\cite{	li2019deep 	}	&	HEVC	&		&	both	&	In-Loop	&		&	L2	&	All QPs	&	QP and CU and TU map	\\
21	&	-	&	APSIPA ASC	-	2019	\cite{	wang2019integrated 	}	&	VVC	&	8	&	Intra	&	Out-Loop	&	DIV2K	&	L2	&	QP-map	&	QP and CU map	\\
27	&	MRRN	&	IEEE-SPL	-	2019	\cite{	 yu2019quality	}	&	HEVC	&		&	both	&	Out-Loop	&	BSDS500	&		&	QP-Specific	&	QP	\\
28	&	RRCNN	&	  IEEE-TCSVT	-	2019	\cite{	zhang2019recursive	}	&	HEVC	&	16	&	Intra	&	In-Loop	&		&	L2	&	QP-map	&	QP	\\
31	&	B-DRRN	&	PCS	-	2019	\cite{	hoang2019b 	}	&	HEVC	&	29	&		&	Out-Loop	&	A video dataset	&	L2	&	QP-Specific	&	QP CU map  Mean map	\\
34	&	CPHER	&	ICIP	-	2019	\cite{	feng2019coding 	}	&	HEVC	&	64	&	AI	&	Out-Loop	&	Vimeo-90K	&	L1	&	QP-Specific	&	QP Prediction information  Unfiltered frame	\\
35	&	WARN	&	ICIP	-	2019	\cite{	chen2019av1 	}	&	AV1	&	50	&	AI, RA	&	In-loop	&	DIV2K 300 videos	&	L2	&	QP-Specific	&	QP	\\
36	&	ACRN	&	ICGIP	-	2019	\cite{	bei2020cu 	}	&	AV1	&	72	&	AI	&	In-loop	&	DIV2K 	&	L2	&	QP-Specific	&	QP	\\
37	&	QG-ConvLSTM	&	ICME	-	2019	\cite{	yang2019quality 	}	&	HEVC	&		&	LD	&	Ou-Loop	&	Vid-70 database	&	L2	&	QP-Specific	&	QP	\\
40	&	ENET-FNET	&	ICCV	-	2019	\cite{	pourreza2019recognizing 	}	&	HEVC	&	24	&		&		&	Kinetics-600	&	L2	&		&		\\
43	&		&	IEEE-TIP	-	2019	\cite{	lu2019deep 	}	&		&		&		&		&		&		&		&		\\
44	&	SimNet	&	PCS	-	2019	\cite{	ding2019cnn 	}	&	AV1	&	25	&	RA	&	In-loop	&	200 videos DIV2K	&	L2	&	QP-Specific	&	QP	\\
45	&	LMVE	&	ICIP	-	2019	\cite{	tong2019learning 	}	&	HEVC	&	20	&	RA	&	Out-loop	&	-	&	L2	&	QP-Specific	&	QP	\\
46	&		&	ICIP	-	2019	\cite{	lu2019learned 	}	&		&		&		&		&		&		&		&		\\
47	&		&	CVPR	-	2019	\cite{	lu2019learned2 	}	&		&		&		&		&		&		&		&		\\
51	&	SEFCNN	&	  IEEE-TCSVT	-	2019	\cite{	ding2019switchable 	}	&	HEVC	&		&	ALL	&	In-Loop	&	DIV2K and a video dataset	&	L2	&	QP-Specific	&	QP	\\
52	&		&	PCS	-	2019	\cite{	xu2019dense 	}	&		&		&		&		&		&		&		&		\\
60	&		&	IEEE-TIP	-	2019	\cite{	jia2019content 	}	&		&		&		&		&		&		&		&		\\
56	&		&	DCC	-	2018	\cite{	wang2018multi 	}	&		&		&		&		&		&		&		&		\\
5	&	-	&	ICIP	-	2018	\cite{	he2018enhancing 	}	&	HEVC	&	69	&	LD	&	Out-Loop	&	-	&	L2	&	QP-specific	&	Partitioning mask Mean-mask	\\
9	&	QECNN-I QECNN-P	&	  IEEE-TCSVT	-	2018	\cite{	yang2018enhancing 	}	&	HEVC	&	9	&	Different network	&	Out-Loop	&	BSDS500	&	L2	&	QP-Specific	&	QP	\\
11	&	Inception module	&	IEEE access	-	2018	\cite{	soh2018reduction 	}	&	HEVC	&	24	&	both	&	Out-Loop	&	JCT-VC	&	L1	&	QP-Specific	&	QP	\\
14	&	MFQE	&	CVPR	-	2018	\cite{	yang2018multi 	}	&	HEVC	&		&	-	&	Out-loop	&	JCT-VC	&	L2	&	QP-Specific	&	QP	\\
20	&	CNNF	&	ICIP	-	2018	\cite{	song2018practical 	}	&		&		&		&		&		&		&		&		\\
23	&	RHCNN	&	IEEE-TIP	-	2018	\cite{	zhang2018residual 	}	&	HEVC	&	19	&	Different	&	In-loop	&	CTC-HEVC	&	L2	&		&		\\
26	&	FECNN	&	ICIP	-	2018	\cite{	li2018deep	}	&	HEVC	&	9	&	Intra	&	Out-Loop	&	BSDS500	&	L2	&	QP-specific	&		\\
29	&	Residual-VRN	&	BigMM	-	2018	\cite{	ma2018residual 	}	&	HEVC	&	15	&	intra	&	Out-Loop	&	MSCOCO	&	L1 + Ms-SSIM	&	QP-Specific	&	QP Residual information  Prediction information	\\
32	&	CNNIF	&	CVPR	-	2018	\cite{	chen2018cnn	}	&	-	&		&		&	In-loop 	&	CLIC	&		&		&		\\
33	&	MGANet	&	arXiv 	-	2018	\cite{	meng2018mganet 	}	&	HEVC	&	16	&	AI, RA, LD	&	Out-Loop	&	Derfs collection1	&	Multi-scale L2	&	QP-specific	&	QP TU map	\\
53	&		&	DCC	-	2018	\cite{	meng2018new 	}	&		&		&		&		&		&		&		&		\\
54	&		&	ICASSP	-	2018	\cite{	jin2018quality 	}	&		&		&		&		&		&		&		&		\\
57	&		&	VCIP	-	2018	\cite{	wang2018dense 	}	&		&		&		&		&		&		&		&		\\
59	&		&	VCIP	-	2018	\cite{	dai2018cnn 	}	&		&		&		&		&		&		&		&		\\
	&		&	ECCV	-	2018	\cite{	lu2018deep 	}	&		&		&		&		&		&		&		&		\\
4	&	STResNet	&	VCIP	-	2017	\cite{	jia2017spatial 	}	&	HEVC	&	4	&	Inter-fix QP in RA	&	In-Loop- signaling on	&	AVS2 test sequences	&	L2	&	QP-specific	&	QP	\\
13	&	DCAD	&	DCC	-	2017	\cite{	wang2017novel 	}	&	HEVC	&	10	&	both	&	Out-Loop	&	-	&	L2	&	QP-Specific	&	QP	\\
55	&	DSCNN	&	ICME	-	2017	\cite{	yang2017decoder 	}	&		&		&		&		&		&		&		&		\\
62	&	CARGAN	&	ICCV	-	2017	\cite{	galteri2017deep	}	&	HEVC	&		&		&		&		&		&		&		\\
65	&	MMS-net	&	ICIP	-	2017	\cite{	kang2017multi 	}	&	HEVC	&	66	&	AI	&	Out-Loop	&	Xiph.org	&	L2- Multi-scale	&	QP-Specific	&	QP CU-TU map	\\
66	&		&	ICCV	-	2017	\cite{	tai2017memnet	}	&		&		&		&		&		&		&		&		\\
67	&	IFCNN	&	IVMSP	-	2016	\cite{	park2016cnn 	}	&	HEVC	&	2	&	both	&	In-loop	&	CTC-test sequences	&	L2	&	QP-specific	&	QP	\\
68	&	NLSLF	&	IEEE-MM 	-	2016	\cite{	ma2016nonlocal 	}	&	HEVC	&		&		&		&		&		&		&		\\

\hline
\hline
\end{tabular}


==> bdrates_PP_AI.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{clccc|ccc||ccc|ccc}
\hline
\hline							
 \multirow{4}{*}{Class} & \multirow{4}{*}{Sequence} & \multicolumn{6}{c||}{CTC QP (22-37)}	& \multicolumn{6}{c}{High QP (32-47)}\\ \cline{3-14}
                       &                     & \multicolumn{6}{c||}{Proposed {(VTM 10.0)}}                  & \multicolumn{6}{c}{Proposed (VTM 10.0)}     \\

                       &                     & \multicolumn{3}{c|}{Without prediction}                      & \multicolumn{3}{c||}{With Prediction}               & \multicolumn{3}{c|}{Without prediction}                                  & \multicolumn{3}{c}{With Prediction} \\

\cline{3-14} 
                       &                        & Y                      & U                      & V                      & Y                      & U                      & V                      & Y                      & U                      & V                      & Y                      & U                      & V                      \\
\hline
\multirow{4}{*}{A1}    & Tango                  & -4.3                   & -4.4                   & -9.1                   & -5.4                   & -21.8                  & -21.1                  & -6.4                   & -10.5                  & -11.9                  & -7.9                   & -20.2                  & -16.9                  \\  
                       & FoodMarket             & -9.9                   & -3.8                   & -9.7                   & -11.3                  & -12.2                  & -13.3                  & -7.8                   & -8.9                   & -10.9                  & -8.8                   & -12.8                  & -11.0                  \\  
                       & CampFire               & -3.3                   & -3.2                   & -11.1                  & -4.0                   & -8.2                   & -20.2                  & -6.4                   & -8.3                   & -11.2                  & -7.6                   & -10.0                  & -18.8                  \\  
                       & \textbf{Average}       & \textbf{-5.8}          & \textbf{-3.8}          & \textbf{-10.0}         & \textbf{-6.9}          & \textbf{-14.1}         & \textbf{-18.2}         & \textbf{-6.9}          & \textbf{-9.3}          & \textbf{-11.3}         & \textbf{-8.1}          & \textbf{-14.4}         & \textbf{-15.6}         \\ 
\hline
\multirow{4}{*}{A2}    & CatRobot               & -5.7                   & -4.7                   & -11.3                  & -6.4                   & -14.0                  & -18.8                  & -6.7                   & -13.1                  & -14.4                  & -8.0                   & -18.0                  & -17.7                  \\  
                       & Daylight               & -2.7                   & -1.7                   & -5.3                   & -3.7                   & -11.9                  & -11.5                  & -7.4                   & -7.9                   & -6.8                   & -8.9                   & -11.9                  & -9.2                   \\  
                       & ParkRunning            & -3.8                   & -0.6                   & -1.6                   & -4.4                   & -4.5                   & -4.4                   & -4.6                   & -2.2                   & -2.3                   & -5.6                   & -5.6                   & -5.3                   \\  
                       & \textbf{Average}       & \textbf{-4.1}          & \textbf{-2.3}          & \textbf{-6.1}          & \textbf{-4.8}          & \textbf{-10.1}         & \textbf{-11.6}         & \textbf{-6.2}          & \textbf{-7.8}          & \textbf{-7.8}          & \textbf{-7.5}          & \textbf{-11.8}         & \textbf{-10.7}         \\ 
\hline
\multirow{6}{*}{B}     & MarketPlace            & -4.2                   & -3.3                   & -7.9                   & -5.2                   & -13.6                  & -14.1                  & -5.2                   & -10.1                  & -11.3                  & -6.5                   & -17.6                  & -15.9                  \\  
                       & RitualDance            & -8.9                   & -4.3                   & -11.4                  & -10.2                  & -14.2                  & -16.9                  & -7.4                   & -9.7                   & -13.8                  & -8.9                   & -17.0                  & -17.4                  \\  
                       & Cactus                 & -4.2                   & -2.1                   & -10.9                  & -4.9                   & -10.2                  & -15.7                  & -6.9                   & -9.9                   & -15.2                  & -8.0                   & -15.3                  & -18.0                  \\  
                       & BasketballDrive        & -5.1                   & -8.2                   & -16.1                  & -6.2                   & -18.9                  & -21.0                  & -6.3                   & -12.8                  & -17.4                  & -7.7                   & -17.9                  & -19.4                  \\  
                       & BQTerrace              & -3.4                   & -4.3                   & -8.2                   & -3.9                   & -13.6                  & -12.5                  & -7.5                   & -9.9                   & -9.4                   & -8.7                   & -15.3                  & -13.7                  \\  
                       & \textbf{Average}       & \textbf{-5.2}          & \textbf{-4.5}          & \textbf{-10.9}         & \textbf{-6.1}          & \textbf{-14.1}         & \textbf{-16.0}         & \textbf{-6.7}          & \textbf{-10.5}         & \textbf{-13.4}         & \textbf{-8.0}          & \textbf{-16.6}         & \textbf{-16.9}         \\ 
\hline
\multirow{5}{*}{C}     & BasketballDrill        & -9.1                   & -11.8                  & -24.3                  & -10.3                  & -23.3                  & -28.0                  & -8.7                   & -19.2                  & -21.2                  & -10.2                  & -21.2                  & -23.0                  \\  
                       & BQMall                 & -6.7                   & -4.5                   & -7.6                   & -7.4                   & -11.7                  & -11.8                  & -7.6                   & -10.4                  & -11.3                  & -8.7                   & -16.9                  & -15.9                  \\  
                       & PartyScene             & -4.4                   & -3.1                   & -6.0                   & -4.8                   & -8.5                   & -10.0                  & -6.6                   & -9.1                   & -9.7                   & -7.5                   & -14.8                  & -15.3                  \\  
                       & RaceHorses             & -3.3                   & -3.6                   & -9.2                   & -3.8                   & -8.1                   & -12.3                  & -4.8                   & -14.0                  & -18.4                  & -5.7                   & -20.4                  & -22.8                  \\  
                       & \textbf{Average}       & \textbf{-5.9}          & \textbf{-5.7}          & \textbf{-11.8}         & \textbf{-6.6}          & \textbf{-12.9}         & \textbf{-15.5}         & \textbf{-6.9}          & \textbf{-13.2}         & \textbf{-15.2}         & \textbf{-8.0}          & \textbf{-18.3}         & \textbf{-19.2}         \\ 
\hline
\multirow{5}{*}{D}     & BasketballPass         & -8.0                   & -8.7                   & -15.7                  & -8.8                   & -18.5                  & -18.0                  & -8.7                   & -14.5                  & -18.4                  & -9.8                   & -19.6                  & -22.1                  \\  
                       & BQSquare               & -6.4                   & -0.5                   & -5.3                   & -6.8                   & -4.6                   & -9.5                   & -8.9                   & -3.0                   & -14.5                  & -9.9                   & -6.1                   & -17.1                  \\  
                       & BlowingBubble          & -5.3                   & -4.2                   & -6.6                   & -5.9                   & -11.5                  & -11.2                  & -6.3                   & -9.2                   & -9.8                   & -7.4                   & -14.8                  & -13.6                  \\  
                       & RaceHorses             & -5.9                   & -6.1                   & -11.7                  & -6.4                   & -12.8                  & -15.3                  & -6.6                   & -11.9                  & -13.7                  & -7.6                   & -17.4                  & -17.4                  \\  
                       & \textbf{Average}       & \textbf{-6.4}          & \textbf{-4.9}          & \textbf{-9.8}          & \textbf{-7.0}          & \textbf{-11.9}         & \textbf{-13.5}         & \textbf{-7.6}          & \textbf{-9.6}          & \textbf{-14.1}         & \textbf{-8.7}          & \textbf{-14.5}         & \textbf{-17.5}         \\ 
\hline
\multirow{4}{*}{E}     & FourPeople             & -8.3                   & -4.1                   & -5.9                   & -9.3                   & -9.6                   & -9.5                   & -8.0                   & -10.6                  & -11.3                  & -9.6                   & -14.9                  & -14.5                  \\  
                       & Johnny                 & -8.2                   & -7.0                   & -10.5                  & -9.4                   & -15.0                  & -13.1                  & -8.3                   & -15.6                  & -15.0                  & -9.5                   & -20.3                  & -16.7                  \\  
                       & KristenAndSara         & -7.4                   & -4.6                   & -8.6                   & -8.2                   & -11.3                  & -12.0                  & -7.8                   & -14.7                  & -12.6                  & -9.0                   & -19.5                  & -15.3                  \\  
                       & \textbf{Average}       & \textbf{-7.9}          & \textbf{-5.2}          & \textbf{-8.3}          & \textbf{-8.9}          & \textbf{-12.0}         & \textbf{-11.5}         & \textbf{-8.0}          & \textbf{-13.6}         & \textbf{-13.0}         & \textbf{-9.4}          & \textbf{-18.2}         & \textbf{-15.5}         \\ 
\hline
\multicolumn{2}{c}{\textbf{All}}                & \textbf{-1.6}          & \textbf{-1.9}          & \textbf{-2.9}          & \textbf{-4.9}          & \textbf{-6.7}          & \textbf{-8.2}          & \textbf{-5.8}          & \textbf{-4.5}          & \textbf{-9.7}          & \textbf{-6.7}          & \textbf{-12.6}         & \textbf{-14.5}          \\ 
\hline
\hline
\end{tabular}


==> bdrates_pp_RA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.15} 
\begin{tabular}{P{0.009\textwidth}C{0.1\textwidth}ccc|ccc||ccc|ccc}
\hline
\hline							
 \multirow{3}{*}{Class} & \multirow{3}{*}{Sequence} & \multicolumn{6}{c||}{\glspl{ctc} QP (22-37)}	& \multicolumn{6}{c}{High QP (27-42)}\\ \cline{3-14}                       

                       &                     & \multicolumn{3}{c|}{Prediction-unaware}                      & \multicolumn{3}{c||}{Prediction-aware}               & \multicolumn{3}{c|}{Prediction-unaware}                                  & \multicolumn{3}{c}{Prediction-aware} \\

\cline{3-14} 
                       &                        & Y                      & U                      & V                      & Y                      & U                      & V                      & Y                      & U                      & V                      & Y                      & U                      & V                      \\
\hline
\multirow{4}{*}{A1} 	&	Tango	        &	-5.6\% 	&	-14.4\%	&	-12.5\%	&	-8.5\%	&	-15.7\%	&	-14.5\%	&	-6.1\%	&	-12.7\%	&	-11.7\%	&	-7.9\%	&	-13.6\%	&	-12.8\%	\\	
                    	&	FoodMarket	    &	-3.6\%	&	-11.4\%	&	-8.4\%	&	-7.2\%	&	-11.5\%	&	-10.5\%	&	-5.8\%	&	-11.6\%	&	-10.0\%	&	-7.7\%	&	-11.7\%	&	-11.0\%	\\	
                    	&	CampFire	    &	-4.3\%	&	-4.2\%	&	-10.8\%	&	-5.9\%	&	-6.9\%	&	-14.2\%	&	-5.9\%	&	-4.3\%	&	-10.6\%	&	-7.4\%	&	-6.8\%	&	-13.6\%	\\	
                    	&	Average	        &	-4.5\%	&	-10.0\%	&	-10.6\%	&	-7.2\%	&	-11.4\%	&	-13.0\%	&	-5.9\%	&	-9.5\%	&	-10.8\%	&	-7.7\%	&	-10.7\%	&	-12.4\%	\\	\hline
\multirow{4}{*}{A2} 	&	CatRobot	    &	-6.9\%	&	-13.3\%	&	-12.8\%	&	-8.5\%	&	-13.6\%	&	-13.5\%	&	-6.8\%	&	-11.0\%	&	-11.5\%	&	-7.8\%	&	-11.2\%	&	-11.2\%	\\	
                    	&	Daylight	    &	-9.3\%	&	-11.3\%	&	-6.1\%	&	-10.8\%	&	-11.5\%	&	-8.6\%	&	-8.1\%	&	-8.8\%	&	-3.9\%	&	-9.0\%	&	-8.8\%	&	-5.1\%	\\	
                    	&	ParkRunning	    &	-3.0\%	&	-2.6\%	&	-3.5\%	&	-4.1\%	&	-2.4\%	&	-4.2\%	&	-3.2\%	&	-2.7\%	&	-3.4\%	&	-4.2\%	&	-2.9\%	&	-3.9\%	\\	
                    	&	Average	        &	-6.4\%	&	-9.1\%	&	-7.5\%	&	-7.8\%	&	-9.2\%	&	-8.8\%	&	-6.1\%	&	-7.5\%	&	-6.3\%	&	-7.0\%	&	-7.6\%	&	-6.7\%	\\	\hline
\multirow{6}{*}{B}  	&	MarketPlace	    &	-4.8\%	&	-7.2\%	&	-8.5\%	&	-5.6\%	&	-8.0\%	&	-9.8\%	&	-4.6\%	&	-5.8\%	&	-9.2\%	&	-5.2\%	&	-6.2\%	&	-10.0\%	\\	
                    	&	RitualDance	    &	-6.0\%	&	-9.0\%	&	-11.3\%	&	-8.0\%	&	-10.6\%	&	-13.4\%	&	-6.2\%	&	-8.0\%	&	-12.5\%	&	-7.6\%	&	-9.0\%	&	-13.8\%	\\	
                    	&	Cactus	        &	-4.2\%	&	-6.3\%	&	-8.5\%	&	-6.0\%	&	-6.3\%	&	-10.2\%	&	-5.5\%	&	-5.9\%	&	-9.3\%	&	-6.7\%	&	-6.0\%	&	-10.3\%	\\	
                    	&	BasketballDrive	&	-5.4\%	&	-6.8\%	&	-13.4\%	&	-7.0\%	&	-10.1\%	&	-15.3\%	&	-5.8\%	&	-2.2\%	&	-13.4\%	&	-7.0\%	&	-9.4\%	&	-14.4\%	\\	
                    	&	BQTerrace	    &	-4.9\%	&	-11.8\%	&	-9.9\%	&	-5.9\%	&	-13.3\%	&	-12.8\%	&	-6.7\%	&	-7.7\%	&	-6.6\%	&	-7.4\%	&	-8.4\%	&	-7.6\%	\\	
                    	&	Average	        &	-5.1\%	&	-8.2\%	&	-10.3\%	&	-6.5\%	&	-9.7\%	&	-12.3\%	&	-5.8\%	&	-5.9\%	&	-10.2\%	&	-6.8\%	&	-7.8\%	&	-11.2\%	\\	\hline
\multirow{5}{*}{C}  	&	BasketballDrill	&	-6.5\%	&	-12.0\%	&	-15.3\%	&	-8.3\%	&	-12.3\%	&	-16.3\%	&	-6.6\%	&	-10.2\%	&	-16.3\%	&	-7.9\%	&	-10.8\%	&	-15.8\%	\\	
                    	&	BQMall	        &	-5.2\%	&	-5.2\%	&	-6.4\%	&	-6.7\%	&	-5.5\%	&	-7.4\%	&	-6.4\%	&	-3.7\%	&	-6.6\%	&	-7.2\%	&	-4.0\%	&	-6.9\%	\\	
                    	&	PartyScene	    &	-5.3\%	&	-4.7\%	&	-7.3\%	&	-6.1\%	&	-4.8\%	&	-8.2\%	&	-5.9\%	&	-3.6\%	&	-6.6\%	&	-6.3\%	&	-3.8\%	&	-6.7\%	\\	
                    	&	RaceHorses	    &	-2.8\%	&	-8.4\%	&	-8.6\%	&	-4.2\%	&	-9.4\%	&	-11.6\%	&	-3.7\%	&	-9.0\%	&	-9.4\%	&	-4.9\%	&	-9.7\%	&	-11.7\%	\\	
                    	&	Average	        &	-5.0\%	&	-7.6\%	&	-9.4\%	&	-6.3\%	&	-8.0\%	&	-10.9\%	&	-5.6\%	&	-6.6\%	&	-9.7\%	&	-6.6\%	&	-7.1\%	&	-10.3\%	\\	\hline
\multirow{5}{*}{D}  	&	BasketballPass	&	-8.0\%	&	-7.5\%	&	-16.6\%	&	-8.9\%	&	-7.9\%	&	-17.2\%	&	-9.0\%	&	-6.3\%	&	-16.8\%	&	-9.4\%	&	-6.8\%	&	-16.8\%	\\	
                    	&	BQSquare	    &	-12.4\%	&	-3.8\%	&	-5.9\%	&	-12.8\%	&	-4.3\%	&	-6.8\%	&	-12.8\%	&	-0.5\%	&	-3.7\%	&	-12.9\%	&	-1.2\%	&	-4.2\%	\\	
                    	&	BlowingBubble	&	-6.2\%	&	-5.3\%	&	-6.6\%	&	-7.0\%	&	-5.9\%	&	-8.4\%	&	-6.6\%	&	-3.6\%	&	-4.7\%	&	-7.5\%	&	-4.3\%	&	-6.2\%	\\	
                    	&	RaceHorses	    &	-5.6\%	&	-8.8\%	&	-8.6\%	&	-7.4\%	&	-9.0\%	&	-10.4\%	&	-5.7\%	&	-7.9\%	&	-8.8\%	&	-7.1\%	&	-8.3\%	&	-9.3\%	\\	
                    	&	Average	        &	-8.0\%	&	-6.4\%	&	-9.4\%	&	-9.0\%	&	-6.8\%	&	-10.7\%	&	-8.5\%	&	-4.6\%	&	-8.5\%	&	-9.2\%	&	-5.2\%	&	-9.1\%	\\	\hline
						\multicolumn{2}{c}{All}	&-5.79\%	&	-8.11\%	&	-9.53\%	&	-7.31\%	&	-8.90\%	&	-11.22\%	&	-6.40\%	&	-6.61\%	&	-9.20\%	&	-7.43\%	&	-7.53\%	&	-10.06\%
\\ 
\hline
\hline
\end{tabular}


==> bdrates_pp_RA_VMAF.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.15} 
\begin{tabular}{P{0.009\textwidth}C{0.1\textwidth}cccc|cccc||cccc|cccc}
\hline
\hline							
 \multirow{3}{*}{Class} & \multirow{3}{*}{Sequence} & \multicolumn{8}{c||}{\glspl{ctc} QP (22-37)}	& \multicolumn{8}{c}{High QP (27-42)}\\ \cline{3-16}                       

                       &                     & \multicolumn{4}{c|}{Prediction-unaware}                      & \multicolumn{4}{c||}{Prediction-aware}               & \multicolumn{4}{c|}{Prediction-unaware}                                  & \multicolumn{4}{c}{Prediction-aware} \\

\cline{3-16} 
                       &                        & Y                      & U                      & V                    & VMAF  & Y                      & U                      & V           & VMAF           
					   & Y                      & U                      & V                      & VMAF & Y                      & U                      & V               & VMAF       \\
\hline
\multirow{4}{*}{A1} 	&	Tango	        &	-5.6\% 	&	-14.4\%	&	-12.5\%	&	-6.4\%  & -8.5\%	&	-15.7\%	&	-14.5\%	& -11.7\% &	-6.1\%	&	-12.7\%	&	-11.7\%	& -6.8\% &	-7.9\%	&	-13.6\%	&	-12.8\%	& -11.8\% \\	
                    	&	FoodMarket	    &	-3.6\%	&	-11.4\%	&	-8.4\%	&	-11.9\% & -7.2\%	&	-11.5\%	&	-10.5\%	& -15.5\% &	-5.8\%	&	-11.6\%	&	-10.0\%	& -12.0\%&	-7.7\%	&	-11.7\%	&	-11.0\%	& -15.5\% \\	
                    	&	CampFire	    &	-4.3\%	&	-4.2\%	&	-10.8\%	&	-9.9\%  & -5.9\%	&	-6.9\%	&	-14.2\%	& -14.2\% &	-5.9\%	&	-4.3\%	&	-10.6\%	& -9.1\% &	-7.4\%	&	-6.8\%	&	-13.6\%	& -12.7\% \\	
                    	&	Average	        &	-4.5\%	&	-10.0\%	&	-10.6\%	&	-9.4\%  & -7.2\%	&	-11.4\%	&	-13.0\%	& -13.8\% &	-5.9\%	&	-9.5\%	&	-10.8\%	& -9.3\% &	-7.7\%	&	-10.7\%	&	-12.4\%	& -13.3\% \\	\hline
\multirow{4}{*}{A2} 	&	CatRobot	    &	-6.9\%	&	-13.3\%	&	-12.8\%	&	-5.4\%  & -8.5\%	&	-13.6\%	&	-13.5\%	& -11.1\% &	-6.8\%	&	-11.0\%	&	-11.5\%	& -5.7\% &	-7.8\%	&	-11.2\%	&	-11.2\%	& -10.9\% \\	
                    	&	Daylight	    &	-9.3\%	&	-11.3\%	&	-6.1\%	&	-9.4\%  & -10.8\%	&	-11.5\%	&	-8.6\%	& -15.4\% &	-8.1\%	&	-8.8\%	&	-3.9\%	& -9.7\% &	-9.0\%	&	-8.8\%	&	-5.1\%	& -15.4\% \\	
                    	&	ParkRunning	    &	-3.0\%	&	-2.6\%	&	-3.5\%	&	-1.4\%  & -4.1\%	&	-2.4\%	&	-4.2\%	& -5.5\%  &	-3.2\%	&	-2.7\%	&	-3.4\%	& -1.8\% &	-4.2\%	&	-2.9\%	&	-3.9\%	& -5.3\%  \\	
                    	&	Average	        &	-6.4\%	&	-9.1\%	&	-7.5\%	&	-5.4\%  & -7.8\%	&	-9.2\%	&	-8.8\%	& -10.7\% &	-6.1\%	&	-7.5\%	&	-6.3\%	& -5.7\% &	-7.0\%	&	-7.6\%	&	-6.7\%	& -10.6\% \\	\hline
\multirow{6}{*}{B}  	&	MarketPlace	    &	-4.8\%	&	-7.2\%	&	-8.5\%	&	-5.0\%  & -5.6\%	&	-8.0\%	&	-9.8\%	& -7.5\%  &	-4.6\%	&	-5.8\%	&	-9.2\%	& -5.2\% &	-5.2\%	&	-6.2\%	&	-10.0\%	& -7.3\%  \\	
                    	&	RitualDance	    &	-6.0\%	&	-9.0\%	&	-11.3\%	&	-8.5\%  & -8.0\%	&	-10.6\%	&	-13.4\%	& -11.7\% &	-6.2\%	&	-8.0\%	&	-12.5\%	& -8.3\% &	-7.6\%	&	-9.0\%	&	-13.8\%	& -11.2\% \\	
                    	&	Cactus	        &	-4.2\%	&	-6.3\%	&	-8.5\%	&	-6.3\%  & -6.0\%	&	-6.3\%	&	-10.2\%	& -8.6\%  &	-5.5\%	&	-5.9\%	&	-9.3\%	& -6.4\% &	-6.7\%	&	-6.0\%	&	-10.3\%	& -8.5\%  \\	
                    	&	BasketballDrive	&	-5.4\%	&	-6.8\%	&	-13.4\%	&	-3.9\%  & -7.0\%	&	-10.1\%	&	-15.3\%	& -7.3\%  &	-5.8\%	&	-2.2\%	&	-13.4\%	& -4.7\% &	-7.0\%	&	-9.4\%	&	-14.4\%	& -7.7\%  \\	
                    	&	BQTerrace	    &	-4.9\%	&	-11.8\%	&	-9.9\%	&	1.3\%   & -5.9\%	&	-13.3\%	&	-12.8\%	& -2.9\%  &	-6.7\%	&	-7.7\%	&	-6.6\%	& 0.1\%  &	-7.4\%	&	-8.4\%	&	-7.6\%	& -3.3\%  \\	
                    	&	Average	        &	-5.1\%	&	-8.2\%	&	-10.3\%	&	-4.5\%  & -6.5\%	&	-9.7\%	&	-12.3\%	& -7.6\%  &	-5.8\%	&	-5.9\%	&	-10.2\%	& -4.9\% &	-6.8\%	&	-7.8\%	&	-11.2\%	& -7.6\%  \\	\hline
\multirow{5}{*}{C}  	&	BasketballDrill	&	-6.5\%	&	-12.0\%	&	-15.3\%	&	-6.4\%  & -8.3\%	&	-12.3\%	&	-16.3\%	& -9.4\%  &	-6.6\%	&	-10.2\%	&	-16.3\%	& -6.4\% &	-7.9\%	&	-10.8\%	&	-15.8\%	& -9.2\%  \\	
                    	&	BQMall	        &	-5.2\%	&	-5.2\%	&	-6.4\%	&	-4.9\%  & -6.7\%	&	-5.5\%	&	-7.4\%	& -8.7\%  &	-6.4\%	&	-3.7\%	&	-6.6\%	& -5.0\% &	-7.2\%	&	-4.0\%	&	-6.9\%	& -8.4\%  \\	
                    	&	PartyScene	    &	-5.3\%	&	-4.7\%	&	-7.3\%	&	-3.9\%  & -6.1\%	&	-4.8\%	&	-8.2\%	& -7.5\%  &	-5.9\%	&	-3.6\%	&	-6.6\%	& -4.0\% &	-6.3\%	&	-3.8\%	&	-6.7\%	& -7.0\%  \\	
                    	&	RaceHorses	    &	-2.8\%	&	-8.4\%	&	-8.6\%	&	-4.0\%  & -4.2\%	&	-9.4\%	&	-11.6\%	& -7.4\%  &	-3.7\%	&	-9.0\%	&	-9.4\%	& -4.1\% &	-4.9\%	&	-9.7\%	&	-11.7\%	& -7.1\%  \\	
                    	&	Average	        &	-5.0\%	&	-7.6\%	&	-9.4\%	&	-4.8\%  & -6.3\%	&	-8.0\%	&	-10.9\%	& -8.2\%  &	-5.6\%	&	-6.6\%	&	-9.7\%	& -4.9\% &	-6.6\%	&	-7.1\%	&	-10.3\%	& -7.9\%  \\	\hline
\multirow{5}{*}{D}  	&	BasketballPass	&	-8.0\%	&	-7.5\%	&	-16.6\%	&	-7.2\%  & -8.9\%	&	-7.9\%	&	-17.2\%	& -10.0\% &	-9.0\%	&	-6.3\%	&	-16.8\%	& -6.7\% &	-9.4\%	&	-6.8\%	&	-16.8\%	& -9.2\%  \\	
                    	&	BQSquare	    &	-12.4\%	&	-3.8\%	&	-5.9\%	&	1.1\%   & -12.8\%	&	-4.3\%	&	-6.8\%	& -2.4\%  &	-12.8\%	&	-0.5\%	&	-3.7\%	& 0.1\%  &	-12.9\%	&	-1.2\%	&	-4.2\%	& -2.8\%  \\	
                    	&	BlowingBubble	&	-6.2\%	&	-5.3\%	&	-6.6\%	&	-7.3\%  & -7.0\%	&	-5.9\%	&	-8.4\%	& -9.2\%  &	-6.6\%	&	-3.6\%	&	-4.7\%	& -6.7\% &	-7.5\%	&	-4.3\%	&	-6.2\%	& -8.4\%  \\	
                    	&	RaceHorses	    &	-5.6\%	&	-8.8\%	&	-8.6\%	&	-6.0\%  & -7.4\%	&	-9.0\%	&	-10.4\%	& -8.3\%  &	-5.7\%	&	-7.9\%	&	-8.8\%	& -5.3\% &	-7.1\%	&	-8.3\%	&	-9.3\%	& -7.3\%  \\	
                    	&	Average	        &	-8.0\%	&	-6.4\%	&	-9.4\%	&	-4.9\%  & -9.0\%	&	-6.8\%	&	-10.7\%	& -7.5\%  &	-8.5\%	&	-4.6\%	&	-8.5\%	& -4.7\% &	-9.2\%	&	-5.2\%	&	-9.1\%	& -6.9\%  \\	\hline
					\multicolumn{2}{c}{All}	&   -5.79\%	&	-8.11\%	&	-9.53\%	&	-5.5\%  & -7.31\%	&	-8.90\%	&	-11.22\%& -9.2\%  &	-6.40\%	&	-6.61\%	&	-9.20\%	& -5.7\% &	-7.43\%	&	-7.53\%	&	-10.06\% & -8.9\%
\\ 
\hline
\hline
\end{tabular}

